Numerical simulation of the response of single gap timing RPCs with the space charge effects and Garfield++

In this article, we report the simulated response of timing RPCs of different gas gaps. A 3D Montecarlo code was developed and integrated with Garfield++ to simulate the avalanche processes with space charge effects which allow actual charge and timing spectrums. The results of this study are presented with examples of timing RPCs of gas gaps 0.02 cm and 0.03 cm.

==> doc/tmp.tex <==
% !TeX root = elsdoc-cas.tex
  \cormark[1]
  \fnmark[1]
  \ead{cvr_1@tug.org.in}
  \ead[url]{www.cvr.cc, www.tug.org.in}

  \credit{Conceptualization of this study, Methodology,
          Software}

  \address[1]{Indian \TeX{} Users Group, Trivandrum 695014,
       India}

  \author[2,4]{Han Theh Thanh}[style=chinese]

  \author[2,3]{T. Rishi Nair}[role=Co-ordinator,
                   suffix=Jr]
  \fnmark[2]
  \ead{rishi@sayahna.org}
  \ead[URL]{www.sayahna.org}

  \credit{Data curation, Writing - Original draft preparation}

  . . .
  . . .
  . . .
  \printcredits

